Evaluating How Developers Use General-Purpose Web-Search for Code Retrieval

Search is an integral part of a software development process. Developers often use search engines to look for information during development, including reusable code snippets, API understanding, and reference examples. Developers tend to prefer general-purpose search engines like Google, which are often not optimized for code related documents and use search strategies and ranking techniques that are more optimized for generic, non-code related information. In this paper, we explore whether a general purpose search engine like Google is an optimal choice for code-related searches. In particular, we investigate whether the performance of searching with Google varies for code vs. non-code related searches. To analyze this, we collect search logs from 310 developers that contains nearly 150,000 search queries from Google and the associated result clicks. To differentiate between code-related searches and non-code related searches, we build a model which identifies the code intent of queries. Leveraging this model, we build an automatic classifier that detects a code and non-code related query. We confirm the effectiveness of the classifier on manually annotated queries where the classifier achieves a precision of 87%, a recall of 86%, and an F1-score of 87%. We apply this classifier to automatically annotate all the queries in the dataset. Analyzing this dataset, we observe that code related searching often requires more effort (e.g., time, result clicks, and query modifications) than general non-code search, which indicates code search performance with a general search engine is less effective.

==> Makefile <==
# $Id: Makefile 1833 2006-06-19 21:51:36Z witchel $

.SUFFIXES: .fig .dvi .ps .pdf

VERSION = 0.0

#----------------------------------------------------------------------
# Source files.  Edit these variables for each new paper.
#----------------------------------------------------------------------

name = main

all: pdf bib

#----------------------------------------------------------------------
# LaTeX commands.
#----------------------------------------------------------------------

%.dvi:%.tex
	pdflatex $<

dvi: $(name).tex *.tex
	pdflatex $<

rub: $(name).tex 
	rubber -Wrefs -Wmisc $(name)

twice:
	pdflatex $(name)
	pdflatex $(name)

bib:
	bibtex $(name)
	pdflatex $(name)
	pdflatex $(name)


latex_junk = 	$(name).dvi \
		*.aux \
		*.log \
		$(name).blg \
		$(name).toc \
		psfig.aux \
		*.bbl \
		*.pdfsync

#----------------------------------------------------------------------
# Postscript/PDF generation.
#----------------------------------------------------------------------

$(name).ps:
ps: $(name).dvi *.tex
	latex $(name).tex && latex $(name).tex
	$(DVIPS) -P pdf -t letter -o $(name).ps $(name).dvi

summary: summary.dvi

#DVIPS = dvips
DVIPS = dvips

%.ps:%.dvi
	$(DVIPS) -P pdf -t letter -o $@ $<

%.ps2:%.dvi
	$(DVIPS) -t letter -o ps2.tmp -p 2 $<
	mpage -2 -P ps2.tmp > $@
	rm ps2.tmp

pdf: 
	pdflatex $(name).tex

# DISTILL = distill
DISTILL_FLAGS = -embedallfonts on -maxsubsetpct 100

DISTILL = ps2pdf
#DISTILL_FLAGS =

%.pdf:%.ps
	$(DISTILL) $(DISTILL_FLAGS) $<

#----------------------------------------------------------------------
# Document previewers.
#----------------------------------------------------------------------

x:
	xdvi -s 5 $(name) &

gv: $(name).ps
	ghostview $(name).ps &


# Garbage files.
junk = $(latex_junk) *.ps *.pdf *.out


#----------------------------------------------------------------------
# Miscellaneous.
#----------------------------------------------------------------------

tags:
	etags $(latex_files)

clean:
	rm -f $(junk)

count:
	wc $(latex_files)

